Performance of Hamamatsu VUV4 SiPMs for detecting liquid argon scintillation

Detection of light signals is crucial to a wide range of particle detectors. In particular, efficient detection of vacuum ultraviolet (VUV) light will provide new opportunities for some novel detectors currently being developed, but is technically challenging. In this article, we characterized the performance of Hamamatsu VUV4 silicon photomultipliers (SiPMs) for detecting VUV argon scintillation light without wavelength shifting. Using a customized cryogenic amplifier design, we operated two models of VUV4 SiPMs inside liquid argon and thoroughly examined their direct sensitivities to liquid argon scintillation. In addition to describing their cryogenic performance, we measured a photon detection efficiency of $14.7^{+1.1}_{-2.4}$% and $17.2^{+1.6}_{-3.0}$% at 128 nm for these two VUV4 models for operation at 4 V of overvoltage, with the main uncertainty arising from the SiPM reflectivity for VUV light.

==> PastTextCopiesOfInterest.tex <==
introduction

% in a comparison between identical SiPM models, one covered with a quartz glass window and one with no window, along with measurements of previously measured properties including argon scintillation's triplet state de-excitation time and prompt-to-total scintillation light ratio. 
%The performance of the Hamamatsu VUV4 S13370 and S13371 SiPMs with on-board amplification in the liquid argon environment is presented.  

%Furthermore, sensitivity across the VUV spectrum is ideal for studying the effects of xenon doping in argon TPCs, a technique currently being explored for combining the best characteristics of both elements into a single detector.  
%However, measurements of the PDE for these VUV4 SiPMs have been made at xenon scintillation wavelengths and found to be lower than that quoted by Hamamatsu.  
%We conducted a similar cross-check of the PDE at the argon scintillation wavelength \cancel{should be conducted} to quantify the performance of these SiPMs for detection of scintillation and ionization signals in dual-phase argon TPCs.    

Instrumental setup section
%Typical Am-241 \jx{-induced liquid argon scintillation} candidate signals have a prompt peak of multiple photoelectrons, followed by a tail of photoelectrons more separated in time.  Features of the average waveform for all candidate Am-241 events were then extracted and utilized to characterize the scintillation light.
%\epb{Put stuff here briefly introducing At light production microphysics...}


%\jk{The mounting cell sits in a vacuum-insulated cryostat which is filled with argon. The cryostat is filled to a certain depth with liquid, and the argon above this depth is in the gas phase. The liquid level of the argon is adjusted such that the mounting cell containing the SiPMs is completely submerged in liquid argon. The benefit of a cryogenic system is that liquid argon is hundreds of times denser than gaseous argon, which increases the interaction rate in the cell.}

%\jk{The argon is sourced from a 99.999\% gas cylinder into a gas panel, which first routes through an MKS GM50A004503R5M020 (shorten to GM50A?) Mass Flow Controller (MFC) and then through a SAES Mono-Torr PS3-MT3-R-1 Getter, which serves as a chemical filler to further purify the argon. The detector-bound argon then flows through the outer chamber of a heat exchanger, which contains two isolated, but thermally-linked, chambers. The inner chamber contains cryogenic argon that is connected to a Suitomo Cryogenics CH-104 copper coldhead that is kept cold by a Suitomo Cryogenics HV-4A2 Zephyr Cryocooler Compressor. The detector-bound argon is cooled by the inner chamber and condenses as it flows down into the base of the main detector bath. This argon circulates through the main bath and heat exchanger through a thermosyphon, but there is no circulation back into the Getter. This means that the argon is only purified once before entry into the main bath. However, no deterioration in the light collection efficiency was observed over the twelve day operation of the teststand. A circulation path will be implemented in future operations to allow for continuous circulation. (What kind of diagram do we want here, if any? Some simplified P&ID? We will already have a picture of the stand.)}

%\jk{A slow control system was implemented with two heaters controlled by PID loops to maintain a vapour pressure in the detector space of $1.500 \pm 0.005$ bar. The coexistence of liquid and vapour at a fixed pressure constrains the temperature at the gas-liquid interface along the boiling curve. (maybe add another sentence: This temperature corresponds to 91.194 K. (I computed this from NIST chemistry webbook; is it necessary to cite?))}

%Direct detection of 128 nm Argon scintillation light
https://www.sciencedirect.com/science/article/pii/S0149197017301610

VUV origin of SiPM signals
%any detected signal in the windowed SiPM should primarily be from photons of longer wavelength than this \cite{Newport}.   Conversely, any light signal measured in the windowless S13371 deviating from the windowed model should result from shorter wavelength light (specifically the 128 nm scintillation emission for liquid argon).

Intro to crosstalk and afterpulsing example
%Performance characteristics of the S13371 and S13370 SiPMs were measured with a combination of Am-241 calibration data and oxygen-quenched argon with no source.  Gain, dark noise, and afterpulsing measurements benefit from having low rates of scintillation event contamination, and are characterized with the oxygen-quenched argon data sets.  On the other hand, even oxygen-quenched data with no source present can still have background events from through-going muons or radioactive backgrounds in the test stand.  As such, crosstalk probabilities are estimated using pulses in the tail of Am-241 calibration data.  Pulses in the late tail of Am-241 events have a low probability of pulse pile-up, reducing systematic errors they introduce when characterizing crosstalk and afterpulsing with single photoelectron (SPE) pulses.  

Cross-talk probability
%The bounds for each value have been shifted from the referenced analysis' [0.5,1.5] PE to better separate single photoelectrons+afterpulsing from all other multi-photoelectron pulses.  
%Note that, although $N_{1.75 PE}/N_{0.75 PE}$ calculates the probability that cross-talk occurs, this is equivalent to how much a single photoelectron is charge-shifted under the assumption that cross-talk is a Poisson process (\jx{can you elaborate? I don't quite understand}).



\begin{comment}
The %mean 
number of photons incident on each SiPM-TIA module is estimated using a Geant4 optical simulation of the teststand and calibration source.  The SiPM cells, PCB boards, mounting cell, and detector can
geometries are all included in the optical simulation, with all surfaces treated as non-reflective except for the SiPM photosensitive areas.  The SiPM phtosensitive areas are assigned a reflectivity of 24\%, based on the simulation's mean photon incident angle on each SiPM and values reported in \cite{nEXO2019jhg} (uncertainty in the SiPM reflectivity is discussed later).  
In the simulation, the Am-241 source is modeled as a point source emitting 59.54 keV gammas at the position outside of the detector can used during calibration, and scintillation photons of 128 nm were generated inside the liquid argon where the gamma energy was deposited.
The absolute light yield of liquid argon used in the simulation is set as
the mean absolute light yield of all data points reported between 30-200 keV in \cite{LArLightYield},
corresponding to a value of $41.1\pm1.2$ photons per keV energy deposited.  
So for every Am-241 gamma ray that deposited full energy in the active liquid argon volume, 2447 primary scintillation photons were generated on average.
%TODO Discuss how the reflectivity is incorporated.  I propose we run the simulation with 31\% reflection probability (measured in \cite{VUV4Reflection}) and apply a systematic based on the difference in the fit mean at 0\% reflection probability (and a higher value?).
\end{comment}


%TODO The below paragraph is going to change.  We should instead use a fit to the distribution, which is exponential + gaussian.  Just calculating the statistical mean for a distribution with more than one Gaussian (there's potentially backgrounds/partial scatters at low PE, which is seen in the simulation as well) isn't right/ideal.  

%In the simulation (calibration) data, the mean number of photons (photoelectrons) detected in Am-241 events is estimated using an exponential + Gaussian fit.  An exponential component is used to model the population of low photon count distribution near zero due to partial energy depositions and events at the edge of the SiPM cell,while the Gaussian component is used to estimate the mean of the Am-241 area distribution hump corresponding tith full Am-241 energy depositions toward the center of the cell volume. Both components can be clearly observed in Figure~\ref{fig:WWLComp} (right). Fits are performed from 0.5 PE to 1.5 times the peak of the Am-241 peak.  

 
% The mean photoelectron fits in calibration data are used to calculate the PDE estimate after applying corrections to the fit mean resulting from crosstalk and afterpulsing.  The equation for calculating the mean number of detected photoelectrons with corrections applied is:

%jx{why should it be expo+gaus? why not Poissionian? And why do we need a fit (can we just calculate the mean)? Is this how you include the 0 PE contribution?}),
% The photon in simulation is in a statistical regime where Poisson and Gaussian should have nearly the same shape.  This may not be the case for the very low overvoltage data points in the S13370 though, as the mean is around 5 PE. I used a fit because I worried that higher energy events in the actual calibration data (double gamma scatters, muons, other possible high energy backgrounds) could bias the statistical mean.

%\begin{equation}
%    \mu_{PE, ^{241}Am}(V) = \frac{\mu_{Q, ^{241}Am}(V)}{G(V) C_{CT}(V) C_{AP}(V)}
%\end{equation}

%Where $\mu_Q$ is the mean or pulse area fit to the Am-241 peak in calibration data, $G(V)$ is the SPE area of the SiPM-TIA, and $C_{CT}(V)$ and $C_{AP}(V)$ are corrections for the mean additional charge measured per photoelectron due to crosstalk and afterpulsing, respectively.   


%measured for each Am-241 run were estimated with the uncertainty on the fit to the Am-241 peak's mean, along with propagated uncertainties on gain, crosstalk, and afterpulsing estimates.   Uncertainties for the gain, crosstalk, and afterpulsing as a function of overvoltage are applied using uncertainties discussed in sections \ref{subsec:Gain} and \ref{subsec:CTAP}.  
%Uncertainties in the mean photoelectrons measured for each Am-241 run were estimated with the uncertainty on the fit to the Am-241 peak's mean, along with propagated uncertainties on gain, crosstalk, and afterpulsing estimates.   Uncertainties for the gain, crosstalk, and afterpulsing as a function of overvoltage are applied using uncertainties discussed in sections \ref{subsec:Gain} and \ref{subsec:CTAP}.


%As a result we calculated the pulse area by scaling up the integrated pulse tail area of [3,9] $\mu s$ based on the average pulse shape. This process introduced an additional uncertainty that was estimated to be 5\%.
%\todo{Look at this correction carefully next week.  Figure out how to apply it properly using the new fit approach.}
% Regarding a saturation correction,  I'm not sure how to do this yet using the fitting approach.For some higher overvoltages on the S13371 and S13370, saturation was observed in the amplifier output signal in the prompt scintillation peak.  The correction was straightforward when just taking the average charge of all events in data (correction factor was linear), but trying to take the ratio of the late window relative to the fit of the Am-241 shoulder is not linear at all (20-30% deviation, exponential-like shape). 

%\begin{equation}
%    \mu_{PE, ^{241}Am}(V) = \frac{\mu_{PE, L ^{241}Am}(V)}{R_L}
%\end{equation}

